Grounded Language Agent for Product Search via Intelligent Web Interactions

The development of agents powered by large language models (LLMs) to accomplish complex high-level user intents, has attracted significant attention recently. However, employing LLMs with billions of parameters (e.g., GPT-4) may incur substantial costs on top of handcrafting extensive prompts. To address this, we introduce a Grounded Language Agent for Intelligent Web Interactions, named GLAINTEL. GLAINTEL employs Flan-T5 as its backbone and is flexible in training in various settings: unsupervised learning, supervised learning, and unsupervised domain adaptation. Specifically, we tackle both the challenge of learning without human demonstrations and the opportunity to leverage human demonstrations effectively when those are available. Additionally, we explore unsupervised domain adaptation for cases where demonstrations are limited to a specific domain. Experimental evaluations across diverse setups demonstrate the effectiveness of GLAINTEL in unsupervised settings, outperforming in-context learning-based approaches that employ larger models with up to 540 billion parameters. Surprisingly, behavioral cloning-based methods that straightforwardly use human demonstrations do not outperform unsupervised variants of GLAINTEL. Additionally, we show that combining human demonstrations with reinforcement learning-based training yields results comparable to methods utilizing GPT-4. The code is available at: https://github.com/MultifacetedNLP/WebAgents-Unsupervised.

==> background.tex <==
\section{Preliminaries}
\subsection{Problem Formulation}
Given a user intent in natural language, the agent's goal is to buy the most appropriate product that fulfills the user's intent.
%
We formulate the task as a goal-augmented Partially Observable Markov Decision Process $\mdp = (\states,\actions,\transitions,\rewardevent,\goal,\observations,\gamma)$, where $\states$ is a set of states $\bs \in \states$;
$\actions \subset \vocabulary^N$ represents action space sampled from LLM's vocabulary $\vocabulary$ of size $N$;
$\goal \subset \vocabulary^N$ denotes the goal space;
$\transitions: \states \times \actions \mapsto \states$ is the transition function;
$\rewardevent: \states \times \actions \times \goal \mapsto \real$ characterizes the goal-conditioned reward function;
$\observations$ is a set of observations $\bo \in \observations$ (\ie~web page state visible to agent);
$\gamma$ is the discount factor.
We employ the language model's head (\ie distribution over the vocabulary) to accommodate the dynamic action space.
This formulation also facilitates directly computing the log probabilities of each action $\ba_i = ( w_0, \cdots, w_{|\ba_i|} )$ sampled from a dynamic action space given the agent's goal $g \in \goal$ and observation $\bo$.



It is important to note that each web page (or observation in RL terminology) presents a unique set of available actions to the agent, which prevents us from learning a probability distribution over the action space as in classification tasks.
For instance, a search page might present user instructions as part of the observation, with allowed actions such as typing an open-ended textual query or pressing the `Search' button.
Conversely, a product detail page offers a different set of actions including `Back to Search', `< Prev', `Description', `Features', `Reviews', `Buy Now', as well as the product-specific variable number of options, \eg `full', `queen' in the case of a web page for a bed frame.
Figure~\ref{fig:intro} shows the observation and action space for the `search result page'.

%\subsection{Instruction Fine-tuned LLMs}

%\subsection{Pre-trained Large Language Models}
%Pre-trained LLMs have proven to be highly effective in a variety of downstream tasks due to their extensive training on large datasets.
%More recently autoregressive sequence models~\cite{brown2020language} have gained popularity, leveraging the decoder stack from the transformer architecture~\cite{vaswani2017attention}.
%The key concept behind autoregressive models is the factorization of any joint distribution over a sequence, denoted as $x = (x_1,...x_L)$,  in the following autoregressive manner:
%$$
%p(x) = \Pi_{i=1}^L p(x_i|x_{<i}).
%$$

%Using this factorization, the process of estimating the density $p(x)$ is simplified to the learning of individual conditional factors $p(x_i|x_{<i})$, which can be easily parameterized using a transformer model.
%The associated objective function, denoted as %$\mathcal{L}_\mathrm{LM}(p)$, can be expressed as:
%$$
%    \mathcal{L}_\mathrm{LM}(p) = \E_{x\sim\data}\left[\sum_{i=1}^L -\log p(x_i|x_{<i})\right].
%$$

%In this work, we employ instruction-finetuned LLM, specifically the Flan-T5~\cite{Chung2022}.

%We provide an overview of the T5 model and outline the instruction fine-tuning process.

%\stitle{T5 model.}
%The T5 model was first introduced in Raffel et al.'s work \cite{raffel2023exploring}. In this work, the author formulated all of the NLU and NLG tasks by converting them to text-to-text tasks. 
%The T5 model~\cite{raffel2019exploring} follows the encoder-decoder framework, aligning with the original transformer architecture~\cite{vaswani2017attention}.
%In the self-supervised pre-training of the T5 model, the objective influenced by masked language modeling and word dropout techniques~\cite{bowman2015generating} is adopted.
%This objective entails masking 15 percent of the input tokens, where consecutive spans of eliminated tokens are replaced with a sentinel token.
%The model is then trained to predict the original tokens that were replaced with these sentinel tokens.


%This architecture of the T5 mode is different from other models like GPT-2 (which employs a decoder-only architecture) and BERT (known for its encoder-only architecture). Moreover, for self-supervised training of the T5 model, an objective inspired by the masked language modeling and word dropout techniques \cite{bowman2015generating} is adopted.
%This objective involves a process where 15 percent of the input tokens are removed and then consecutive spans of removed tokens are replaced with a sentinel token. Subsequently, the model is trained to predict the original tokens that have been substituted with these sentinel tokens.

%\stitle{Instruction Finetuning.}
%Instruction finetuning is a technique designed to customize LLMs, enabling them to execute specific tasks guided by explicit natural language instructions~\cite{Chung2022}.
%The instruction finetuned variant of T5, called Flan-T5, underwent finetuning using a dataset that encompassed a total of 1836 diverse tasks. 
%This dataset was curated by consolidating information from previous studies, incorporating contributions from T0-SF \cite{sanh2022multitask}, Muffin \cite{wei2022finetuned}, NIV2 \cite{wang-etal-2022-super}, and chain of thought~(CoT).
%Flan-T5 has shown state-of-the-art performance across a range of challenging benchmark such as MMLU~\cite{hendrycks2021measuring}, BBH~\cite{srivastava2023imitation}, TyDiQA~\cite{clark-etal-2020-tydi}, and MGSM~\cite{shi2022language}. 


%was fine-tuned using a dataset comprising a total of 1836 unique tasks was created by aggregating data from prior works, including T0-SF \cite{sanh2022multitask}, Muffin \cite{wei2022finetuned}, NIV2\cite{wang-etal-2022-super}, and CoT (Chain of Thought). 





%As outlined in Chung et al.'s research \cite{Chung2022}, a wide range of models, including T5 and PaLM models, underwent instruction-based fine-tuning. To facilitate this fine-tuning process, a dataset comprising a total of 1836 unique tasks was created by aggregating data from prior works, including T0-SF \cite{sanh2022multitask}, Muffin \cite{wei2022finetuned}, NIV2\cite{wang-etal-2022-super}, and CoT (Chain of Thought). 
%Following this fine-tuning phase, the model's performance was evaluated across four challenging benchmark evaluations: MMLU \cite{hendrycks2021measuring}, BBH \cite{srivastava2023imitation}, TyDiQA \cite{clark-etal-2020-tydi}, and MGSM\cite{shi2022language}. 



%In this work, we employ Flan-T5 as the backbone model and further customize it for our task.
%we took advantage of the Flan-T5 model.
%Specifically, we use the publicly released checkpoints of the Flan-T5 model \footnote{Checkpoints: \href{https://github.com/google-research/t5x/blob/main/docs/models.md\#flan-t5-checkpoints}{https://github.com/google-research/t5x/ blob/main/docs/models.md\#flan-t5-checkpoints}}.

%the checkpoints of the flan-T5 model are publicly released on Google's research Github 

\subsection{Reinforcement Learning}
Reinforcement learning is an extensively studied area in the domain of unsupervised learning.
RL algorithms, such as PPO, have been shown to empower an agent to learn effective decision-making skills in a defined environment, ultimately resulting in the desired outcomes.
To optimize such an agent, methods utilizing policy gradients commonly entail the computation of a gradient estimator, which is subsequently incorporated into a stochastic gradient ascent algorithm.
A common optimization objective for enhancing the policy $\pi$ involves maximizing the expected reward $r \in \mathbb{R}$ over selected action $\ba$ given current state $\bs$.
%
%a generated sequence $\mathbf{Y} = (y_1, \cdots, y_n)$ with a length of $n$. This sequence is produced given an input sequence $\mathbf{X} = (x_1, \cdots, x_m)$ with a length of $m$, sampled from the data distribution $\mathcal{D}$. The optimization of the expected reward can be expressed as:
%\[ \mathbb{E}_{\pi}[r] = \mathbb{E}_{x \sim \mathcal{D}, y \sim \pi(\cdot | x)} [r(x, y)] \]
%
%RL algorithms (\eg PPO) enable an agent to acquire the skill of making decisions within a given environment, ultimately leading to rewarding outcomes.
%This process involves the agent learning a specific task through a series of trials and errors. 
%It gradually knows which actions to take based on its current state, with the ultimate goal of achieving a desired reward at the end of each episode. As the agent continues to learn through this trial-and-error process, it becomes increasingly proficient at selecting the right actions to follow instructions and earn rewards. 
%
%Reinforcement learning algorithms (such as proximal policy optimization, )  This process involves the agent learning a specific task through a series of trials and errors. 
%It gradually knows which actions to take based on its current state, with the ultimate goal of achieving a desired reward at the end of each episode. As the agent continues to learn through this trial-and-error process, it becomes increasingly proficient at selecting the right actions to follow instructions and earn rewards. 
%
%Methods that use policy gradients compute an estimator of the gradient and then plug it into a stochastic gradient ascent algorithm.
%It is common to optimize the policy $\pi$ by maximizing the expected reward $r \in \real$ for the generated sequence $\bigY = (y_1, \cdots, y_n)$ with length $n$, given the input sequence $\bigX = (x_1, \cdots, x_m) $ with length $m$, that is sampled from data distribution $\data$. We can optimize the expected reward as follows:
%$$
%\mathbb{E}_{\pi}[r] = \mathbb{E}_{x \sim \data, y \sim \pi(\cdot | x)} [r(x, y)]
%$$
%
The PPO algorithm introduces a clipped surrogate objective along with a penalty on the KL divergence.
Unlike trust region policy optimization algorithms~\cite{schulman2015trust}, where the Kullback–Leibler~(KL) divergence is imposed as a hard constraint, PPO modifies the objective function using a penalty term associated with KL divergence. 
The policy update in PPO, at step $t$, is given by:
\begin{equation*}
\theta_{t+1} = \arg\max_\theta \mathbb{E}_{\bs, \ba \sim \pi_{\theta_t}} [ \mathcal{L} (\bs, \ba, \theta_t, \theta)]
\end{equation*} 
where $\bs$ represents the state and $\bs$ denotes the action.



%The PPO algorithm introduced clipped surrogate objective, in addition to, the penalty on the KL divergence.
%The objective function is modified using the KL divergence penalty, instead of making it a hard constraint like in the trust region policy optimization algorithms~\cite{schulman2015trust}. The PPO updates its policy, at step $k$ via:
%$$
%\theta_{k+1} = \arg\max_\theta \mathbb{E}_{s,a \sim \pi_{\theta_k}} [ \mathcal{L} (s, a, \theta_k, \theta)]
%$$ 

%In this work, we employ PPO algorithm~\cite{baselines} to perform policy gradients, that has been shown to be scalable (e.g., for large language models), data-efficient, and robust (i.e., without excessive hyperparameter tuning)~\cite{bellemare2013arcade}. 




In our work, we utilize the PPO algorithm~\cite{baselines} for updating the policy of the agent.
This algorithm has demonstrated scalability, particularly in the context of LLMs, as well as efficiency in handling data and robustness without necessitating excessive hyperparameter tuning~\cite{bellemare2013arcade}.



==> trainingDetails.tex <==
\subsection{Implementation Details}


Our implementation operates on a client-server architecture, with the training scripts serving as the client and communicating requests to LLM servers.
Specifically, a master server manages these requests, distributing them across multiple LLM servers.
Once each LLM server completes its computations, the master server consolidates the results and sends them back to the training script.
Furthermore, we use vertical model parallelism, enabling the parallelization of individual LLMs across multiple GPUs.
In our experiments, we utilized a single LLM, Flan-T5-Large, with 780 million parameters.
This model was parallelized across 4 Nvidia V100 32GB GPUs.
We incorporated the last two observations as the model input and an encoder context size of 1024. 



To train the agent using the human demonstrations, we used the Trainer library provided by Huggingface \footnote{Trainer: \href{https://huggingface.co/docs/transformers/main_classes/trainer}{https://huggingface.co/docs/transformers /main\_classes/trainer}}. 
We employed the Adam optimizer, and for the remaining hyperparameter values, refer to Table~\ref{SL_hyperparameters}.
In our unsupervised learning phase, we leverage the PPO algorithm, and the complete values of hyperparameters can be found in Table~\ref{PPO_hyperparameters}.


\begin{table}[t!]
    \centering
    \caption{Supervised Learning Hyperparameters.}
    \vspace{-10pt}
    \begin{tabular}{c|c}
        \toprule
        Hyperparameter & Value \\
        \hline
        Number of Epochs & 10 \\
        Learning Rate & $2 \times 10^{-5}$ \\
        Warmup Steps & 100 \\
        Weight Decay & 0.01  \\
        Batch Size & 32 \\
        Adam Optimizer Epsilon & $10^{-8}$ \\ 
        Adam Optimizer $\beta_1$ & 0.9 \\
        Adam Optimizer $\beta_2$ & 0.999 \\ 
        \bottomrule
    \end{tabular}
    \label{SL_hyperparameters}
    \vspace{-4pt}
\end{table}




\begin{table}[t!]
    \centering
    \caption{Unsupervised Learning Hyperparameters.}
    \vspace{-10pt}
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{c|c}
        \toprule
        Hyperparameter & Value \\
        \hline
        \# of collected transitions between two updates & 640 (16 × 40) \\
        Number of epochs per update & 1 \\ 
        Batch Size & 8 \\
        Learning Rate & $10^{-6}$ \\
        Adam Optimizer Epsilon & $10^{-5}$ \\ 
        Adam Optimizer $\beta_1$ & 0.9 \\
        Adam Optimizer $\beta_2$ & 0.999 \\ 
        Discount Factor & 0.99 \\
        Lambda for Generalized Advantage Estimate & 0.99 \\
        Entropy Loss Coefficient & 0.01 \\
        Value Loss Coefficient & 0.5 \\
        Maximum Gradient Norm & 0.5 \\
        Clipping Epsilon & 0.2 \\
        \bottomrule
    \end{tabular}
    }
    \label{PPO_hyperparameters}
\end{table}




